Recognizing Birds from Sound - The 2018 BirdCLEF Baseline System

Reliable identification of bird species in recorded audio files would be a transformative tool for researchers, conservation biologists, and birders. In recent years, artificial neural networks have greatly improved the detection quality of machine learning systems for bird species recognition. We present a baseline system using convolutional neural networks. We publish our code base as reference for participants in the 2018 LifeCLEF bird identification task and discuss our experiments and potential improvements.

==> textsnippets.tex <==
% rimar: Vorschläge

\subsubsection{Inferences by Sequences}\label{sqgroups}
In a second step we can make use of the sequences. A sequence describes a continued sequence of shots taking place at the same location and time, comparable to scene. We conclude every item of the result that all members of its sequence are depicting the same location, even if it has not been recognized. This is very helpful on shots with strange camera angles and close-ups. All members of the sequence are examined again if person X has been recognized. If so, the shot is added to the result list.
